Clustering and analysis of user behaviour in blockchain: A case study of Planet IX

Decentralised applications (dApps) that run on public blockchains have the benefit of trustworthiness and transparency as every activity that happens on the blockchain can be publicly traced through the transaction data. However, this introduces a potential privacy problem as this data can be tracked and analysed, which can reveal user-behaviour information. A user behaviour analysis pipeline was proposed to present how this type of information can be extracted and analysed to identify separate behavioural clusters that can describe how users behave in the game. The pipeline starts with the collection of transaction data, involving smart contracts, that is collected from a blockchain-based game called Planet IX. Both the raw transaction information and the transaction events are considered in the data collection. From this data, separate game actions can be formed and those are leveraged to present how and when the users conducted their in-game activities in the form of user flows. An extended version of these user flows also presents how the Non-Fungible Tokens (NFTs) are being leveraged in the user actions. The latter is given as input for a Graph Neural Network (GNN) model to provide graph embeddings for these flows which then can be leveraged by clustering algorithms to cluster user behaviours into separate behavioural clusters. We benchmark and compare well-known clustering algorithms as a part of the proposed method. The user behaviour clusters were analysed and visualised in a graph format. It was found that behavioural information can be extracted regarding the users that belong to these clusters. Such information can be exploited by malicious users to their advantage. To demonstrate this, a privacy threat model was also presented based on the results that correspond to multiple potentially affected areas.

==> biography.tex <==

% Biography
\bio{images/dora.jpg}
 \textbf{Dorottya Zelenyanszki:} is a PhD candidate at the School of Information and Communication Technology at Griffth University, Gold Coast, Australia. Her research interests are blockchain, user behaviour and privacy.
\endbio

\bio{images/Zhe.png}
\textbf{Zh\'e H\'ou:} is a Lecturer at Griffith University, Australia. He obtained his Ph.D. degree from the Australian National University in 2015. His research mainly focuses on automated reasoning, formal methods, autonomous systems, machine learning, and blockchain. 
\endbio

\bio{images/KB.jpg}
 \textbf{Kamanashis Biswas:} received his M.Sc. in Computer Science with specialisation in Security Engineering from Blekinge Institute of Technology (BTH), Sweden and Ph.D. in Information and Communication Technology from Griffith University, Australia. Currently, he is working as a Senior Lecturer in Information Technology (Cybersecurity) at Australian Catholic University. Before starting his role at ACU, he worked as an Associate Lecturer at Griffith University for one and a half years. He also worked as a faculty at Daffodil International University, Bangladesh for about four and a half years. His research interests include blockchain technology, privacy issues in the metaverse, explainable AI, design and development of lightweight security protocols, energy efficient and secure routing, intrusion detection systems, and security issues in SDNs, MANETs, and WSNs. He has published numerous papers in the areas of blockchain, WSN, security, and privacy in reputed venues and high-impact journals including IEEE Internet of Things, Computer Networks, Journal of Network and Computer Applications, Future Generation Computer Systems, and Nature Scientific Report. He has served in different leading capacities, such as a keynote speaker, general chair, session chair, organising committee member and/or TPC member of several international conferences including TrustCom, GridCom, SDLT, CISIS, ICCS, ACM BlockSys, and PRDC-23. Dr Biswas has been a recipient of several internal and external research grants. He has also been editor of special issues in international journals and organised several workshops in the past.
\endbio

\bio{images/Photo_Muthu.jpg}
\textbf{Vallipuram Muthukkumarasamy:} received a Ph.D. degree from Cambridge University, England, and a B.Sc.Eng. (Hons.) from the University of Peradeniya, Sri Lanka. He is currently attached to the School of ICT, Griffith University, Australia, as Professor. His research areas include cyber security, blockchain technology, and wireless sensor networks. He has pioneered the Network Security and Blockchain Research Group at the Institute for Integrated and Intelligent Systems. 
\endbio
